WebAssembly Diversification for Malware Evasion

WebAssembly has become a crucial part of the modern web, offering a faster alternative to JavaScript in browsers. While boosting rich applications in browser, this technology is also very efficient to develop cryptojacking malware. This has triggered the development of several methods to detect cryptojacking malware. However, these defenses have not considered the possibility of attackers using evasion techniques. This paper explores how automatic binary diversification can support the evasion of WebAssembly cryptojacking detectors. We experiment with a dataset of 33 WebAssembly cryptojacking binaries and evaluate our evasion technique against two malware detectors: VirusTotal, a general-purpose detector, and MINOS, a WebAssembly-specific detector. Our results demonstrate that our technique can automatically generate variants of WebAssembly cryptojacking that evade the detectors in 90% of cases for VirusTotal and 100% for MINOS. Our results emphasize the importance of meta-antiviruses and diverse detection techniques, and provide new insights into which WebAssembly code transformations are best suited for malware evasion. We also show that the variants introduce limited performance overhead, making binary diversification an effective technique for evasion.

==> dataset.bck.tex <==

%\renewcommand\arraystretch{1.00}


\renewcommand\arraystretch{1.20}

\begin{tabularx}{\linewidth}{l|l ll  lp{0.34\linewidth}}
    \toprule
    
        \textbf{ID}  & \textbf{S} & \textbf{\#I.} & \textbf{\#F.} & \textbf{\#D}  & \textbf{Origin} \\
\hline
% Result from VT
9d30e7f0  & 68796 & 30768 & 61 & 30  & http archive \\

% "Monero miner"
8ebf4e44  & 68803 & 30768 & 61 & 26 & Web crawling \\

47d29959 &  68796 & 30768 & 61 & 31 & \url{https://github.com/davbo/yara-rs/tree/master/sample-miners} \\

% "Crytonight Miner"
\child aafff587  
% cryptonight obfuscated add to the description of the group 
& 97551 & 47033 & 72 & 6 & \url{https://github.com/wenhao1006/SEISMIC/tree/master/CoinHive/64-bit}  \\ 




dc11d82d  & 67496 & 30246 & 49 & 20 & MinerRay \footnotemark[2],  \live \url{http://topfilmonline.ru} \\


% 64bits worker
0d996462 &  70972 & 30531 & 30 & 19  & SEISMIC, MinerRay \live \url{http://filelar.com} \\

% 64bits worker instrumented

\child fbdd1efa  & 94270 & 45905 & 40 & 18 &  \url{https://github.com/wenhao1006/SEISMIC/tree/master/CoinHive/32-bit} \\

\child a32a6f4b & 94461 & 45940 & 40 & 18 &  \url{https://github.com/wenhao1006/SEISMIC/tree/master/CoinHive/64-bit}  \\

 d2141ff2  & 70111 & 31783 & 30 & 9 & MinerRay, SEISMIC \\
 
 046dc081  & 74099 & 31783 & 29 & 6 &  MinerRay, SEISMIC \\
 


24aae13a   & 62458 & 28339 & 37 & 4 &  SEISMIC \\

000415b2   
%    cryptonight obfuscated TODO check, this can be possibly merge with another group 
& 62466 & 28339 & 37 & 3  & SEISMIC \\



643116ff   & 73010 & 31866 &  & 6 & MinerRay  \\


    006b2fb6   & 87502 & 39544 & 90 & 4 & \url{https://github.com/deepwn/deepMiner} \\
    
    
15b86a25   & 100755 & 45881 & 79 & 4 &  MinerRay \\


4cbdbbb1  
%NFWebMiner add to the description
% https://minero.cc/
& 104666 & 47916 & 62 & 3 & \url{https://github.com/wenhao1006/SEISMIC/tree/master/NFWebMiner}  \\

\child 119c53eb  & 137320 & 67069 & 79 & 2   & \url{https://github.com/wenhao1006/SEISMIC/tree/master/NFWebMiner}  \\


f0b24409 & 77572 & 34918 & 59 & 2 & MinerRay   \\

c1be4071 & 77572 & 34918 & 59 & 2 & MinerRay    \\

a74a7cb8 & 77572 & 34918 & 59 & 2 & MinerRay    \\

a27b45ef & 77572 & 34918 & 59 & 2 & MinerRay     \\

6b8c7899 & 77572 & 34918 & 59 & 2 & MinerRay   \\

68ca7c0e & 77572 & 34918 & 59 & 2 & MinerRay     \\

65debcbe & 77572 & 34918 & 59 & 2 & MinerRay    \\

5bc53343 & 77572 & 34918 & 59 & 2 & MinerRay    \\

59955b4c & 77572 & 34918 & 59 & 2 & MinerRay    \\


942be4f7    & 103520 & 46208 & 79 & 4 & MinerRay \\


fb15929f   & 77054 & 33562 & 112 & 4 &  MinerRay  \\


7c36f462   & 121931 & 55839 & 79 & 4 &  MinerRay \\


89a3645c   & 75003 & 34134 & 58 & 2 &  MinerRay \\


dceaf65b    
% cryptonight-(v1|v7)  Check that this is packaged with multiple versions
& 77575 & 34901 & 58 & 2 &   MinerRay  \\


089dd312   
% cryptonight-(v1|v7)  Check that this is packaged with multiple versions
& 79883 & 34989 & 58 & 2 & MinerRay,  \live \url{http://theroyalforums.com},  \live \url{http://prylive.com.meta}  \\


e09c32c5  
%cryptonight (only \_cryptonight\_hash function) Check this 
& 71955 & 32416 & 46 & 1 & MinerRay  \\


\end{tabularx}

==> discussion.tex <==

\section{Discussion}
In this section we mention some challenges we face during the writing of this work.
We enumerate them in order to enforce the debase and the discussion on the topic.

\emph{Oracle classification moves in time:}
One could expect that the more detectors a binary has, the more iterations are needed to evade them.
However, we have observed that this is not the case for some binaries.
The main reason is that the final labelling of binaries for VirusTotal vendors is not immediate \cite{251586}. 
For example, a VirusTotal vendor could label a binary as benign and change it later to malign after several weeks in a conservative way of acting.
This phenomenon creates a time window in which slightly changed binaries (fewer iterations in our case) could evade the detection of numerous vendors.

\emph{Lack of bigger picture:} A WebAssembly cryptomalware can only exist with its JavaScript complement.
For example, a browser cryptonalware needs to send the calculated hashes to a cryptocurrency service.
This network communication is outside the WebAssembly accesses and needs to be delegated to a JavaScript code.
Besides, other functionalities can be intermixing between JavaScript and WebAssembly and in some cases be completely in one side or the other \cite{romano2022wobfuscator}.
This intermixing between JavaScript and WebAssembly could provide statically different WebAssembly. 
% What we saw
We have observed that, the imports and the memory data of the WebAssembly binaries have a high variability in our original dataset.
The imported functions from JavaScript change from binary to binary.
Their data segments can also differ in content and length.
To completely analyze these cases, the whole JavaScript-WebAssembly program is needed, something only provided in 9/33 cases of our dataset.

\emph{More narrowed fitness function:} We use a simple fitness function, but the MCMC evasion algorithm could have a fitness function as general as wanted.
In our case, we do not use binary metadata, instead we focus on the result from the malware oracle, given that the main goal is to evade this oracle.

\emph{Mitigation: } \todo{TBD, data augmentation, better resilience evaluation ?}


Another interesting thing would be to see if there is difference in the detectors. If some detectors are fooled by some transformations or are more robust, etc.

==> old/table-rq2.od.tex <==

\large

\renewcommand\arraystretch{1.50}
\begin{adjustbox}{width=1\linewidth}
    \begin{tabular}{p{1.2cm}|rrr|ccc|ccc}
\textbf{Hash} &  \multicolumn{3}{c|}{\textbf{Baseline}} &  \multicolumn{3}{c|}{\textbf{ME. mcmc}}  & \multicolumn{3}{c}{\textbf{Stacked mutations}} \\
  & \textbf{\#D} & MT. & ME. & 01 & 0.3 & 1.1 & 01 & 0.3 & 1.1 \\
\hline
47d29959 & 31 &  & 26 &  19 & 12 & 10 &   &  &   \\
9d30e7f0 & 30 &  & 24 &  17 & 9 & 10 &   &  &   \\
8ebf4e44 & 26 &  & 21 &  13 & 5 & 4 &   &  &   \\
\hline
dc11d82d & 20 & \textbf{355} & 20 &  20 & 14 & 15 &  444/446 &  &   \\
0d996462 & 19 & \textbf{401} & 19 &  19 & 14 & 4 &  696/697 &  &   \\
a32a6f4b & 18 & 635 & 18 &  18 & 6 & 1 &  \textbf{621/625} &  &   \\
fbdd1efa & 18 & \textbf{310} & 18 &  18 & 3 & 3 &  725/726 &  &   \\
d2141ff2 & 9 & \textbf{461} & 9 &  9 & 9 & 5 &  775/781 & 603/783 &   \\
aafff587 & 6 & 484 & 6 &  2 & 6 & 6 &   & 228/331 & \textbf{76/413}  \\
046dc081 & 6 & 404 & 6 &  6 & 6 & 5 &  397/397 & \textbf{158/159} &   \\
643116ff & 6 & \textbf{144} & 6 &  6 & 6 & 1 &  436/436 & 484/631 &   \\
15b86a25 & 4 & 253 & 4 &  4 & 4 & 4 &  207/208 & 186/214 & \textbf{109/131}  \\
006b2fb6 & 4 & \textbf{282} & 4 &  4 & 4 & 3 &  379/380 & 500/709 &   \\
942be4f7 & 4 & 200 & 4 &  4 & 4 & 4 &  200/200 & 195/200 & \textbf{142/219}  \\
7c36f462 & 4 & 236 & 4 &  4 & 2 & 0 &  \textbf{221/221} &  &   \\
fb15929f & 4 & \textbf{297} & 4 &  2 & 4 & 3 &   & 446/475 &   \\
24aae13a & 4 & \textbf{252} & 4 &  4 & 4 & 3 &  398/401 & 286/446 &   \\
000415b2 & 3 & 302 & 3 &  3 & 3 & 2 &  373/376 & \textbf{19/34} &   \\
4cbdbbb1 & 3 & 295 & 3 &  3 & 3 & 3 &  204/204 & 62/72 & \textbf{168/685}  \\
65debcbe & 2 & 131 & 2 &  2 & 2 & 2 &  33/33 & \textbf{31/33} & 31/33  \\
59955b4c & 2 & 130 & 2 &  2 & 2 & 2 &  \textbf{33/33} & \textbf{33/33} & \textbf{33/33}  \\
89a3645c & 2 & 431 & 2 &  2 & 2 & 2 &  318/319 & 152/197 & \textbf{1/107}  \\
a74a7cb8 & 2 & 124 & 2 &  2 & 2 & 2 &  \textbf{33/33} & \textbf{33/33} & \textbf{33/33}  \\
119c53eb & 2 & 104 & 2 &  2 & 2 & 2 &  44/45 & 352/480 & \textbf{7/18}  \\
089dd312 & 2 & 153 & 2 &  2 & 2 & 2 &  166/166 & 149/167 & \textbf{18/123} \\
c1be4071 & 2 & 130 & 2 &  2 & 2 & 2 &  \textbf{33/33} & \textbf{33/33} & \textbf{33/33} \\
dceaf65b & 2 & 140 & 2 &  2 & 2 & 2 &  165/166 & 165/166 & \textbf{48/132 } \\
6b8c7899 & 2 & 143 & 2 &  2 & 2 & 2 &  \textbf{33/33} & \textbf{33/33} & \textbf{33/33} \\
a27b45ef & 2 & 145 & 2 &  2 & 2 & 2 &  33/33 & \textbf{30/33} & 33/33  \\
68ca7c0e & 2 & 137 & 2 &  2 & 2 & 2 &  33/33 & 121/167 & \textbf{15/595}  \\
f0b24409 & 2 & 127 & 2 &  2 & 2 & 2 &  11/11 & 33/33 & \textbf{11/11}  \\
5bc53343 & 2 & 118 & 2 &  2 & 2 & 2 &  \textbf{33/33} & \textbf{33/33} & \textbf{33/33} \\
e09c32c5 & 1 & \textbf{120} & 1 &  1 & 1 &  &  478/488 & 595/921 &   \\
\end{tabular}

\end{adjustbox}

==> old/table_dataset1.tex <==

%\renewcommand\arraystretch{1.00}

\newenvironment{grouptableheader}[1]
    {
    \begin{tabular}{
        %hash
        p{0.12\linewidth} |
        % description
        %p{0.1\linewidth}
        % size
        p{0.05\linewidth} 
        % #inst
        p{0.06\linewidth} 
        % #Func
        p{0.04\linewidth} 
        % #detectors
        p{0.01\linewidth} 
        % U labels
        %p{0.3\linewidth} 
        % Origin
        p{0.34\linewidth}
        % Live
        % p{0.05\linewidth}
        % MV
       % p{0.05\linewidth}
    }
        
        \textbf{ID}  & \textbf{S} & \textbf{\#I.} & \textbf{\#F.} & \textbf{\#D}  & \textbf{Origin} 
        %& \textbf{Live} 
        % & \textbf{Multivariant}
         \\
    \hline\hline}
    {
    \end{tabular}}
    

\newenvironment{grouptable}[1]
    {
    \begin{tabular}{
    %hash
    p{0.12\linewidth} |
        % description
        %p{0.1\linewidth}
        % size
        p{0.05\linewidth} 
        % #inst
        p{0.06\linewidth} 
        % #Func
        p{0.04\linewidth} 
        % #detectors
        p{0.01\linewidth} 
        % U labels
        %p{0.3\linewidth} 
        % Origin
        p{0.34\linewidth}
        % Live
       %  p{0.05\linewidth}
        % Multivariant
        %p{0.05\linewidth}
    } }
    {
    \end{tabular}}



\begin{grouptableheader}{G1}

% Result from VT
9d30e7f0  & 68796 & 30768 & 61 & 30  & http archive \\
\hline
% "Monero miner"
8ebf4e44  & 68803 & 30768 & 61 & 26 & Web crawling \\
\hline
47d29959 &  68796 & 30768 & 61 & 31 & \url{https://github.com/davbo/yara-rs/tree/master/demo} \\
\hline
% "Crytonight Miner"
\child aafff587  
% cryptonight obfuscated add to the description of the group 
& 97551 & 47033 & 72 & 6 & \url{https://github.com/wenhao1006/SEISMIC/tree/master/CoinHive/64-bit}  \\ 
\hline

% "Miner on the web"
%\begin{comment}
%not-a-virus:risktool.wasm.miner.d
%	wasm.s.coinminer.68803
%	wasm/coinminer.b\_potentially\_unwanted
%	malware.generic-script.save.6e95479e
%	bitcoinminer\_(pua)
%	coinminer\_cryptonight.sm-wasm
%	detected
%	misc.riskware.js.coinminer
%	riskware/coinminer
%	application.bitcoinminer.aam\_(b)
%	miner.wasmwebcoin
%	malware\_(ai\_score=91)
%	wasm/cryptonight
%	generic.application.coinminer.az
%	application.bitcoinminer.aam
%	other:malware-gen\_[trj]
%	wasm/cryptojs
%	riskware.wasm.miner.1!c
%	pua.wasm.coinminer
% \end{comment}

\end{grouptableheader}

\begin{grouptable}{G2} 
dc11d82d  & 67496 & 30246 & 49 & 20 & MinerRay,  \live \url{http://topfilmonline.ru} \\
\hline
\end{grouptable}


\begin{grouptable}{G3}
% 64bits worker
0d996462 &  70972 & 30531 & 30 & 19  & SEISMIC, MinerRay \live \url{http://filelar.com} \\
\hline
% 64bits worker instrumented

\child fbdd1efa  & 94270 & 45905 & 40 & 18 &  \url{https://github.com/wenhao1006/SEISMIC/tree/master/CoinHive/32-bit} \\
\hline
\child a32a6f4b & 94461 & 45940 & 40 & 18 &  \url{https://github.com/wenhao1006/SEISMIC/tree/master/CoinHive/64-bit}  \\
\hline
 d2141ff2  & 70111 & 31783 & 30 & 9 & MinerRay, SEISMIC 32-bit  \\
 \hline
 046dc081  & 74099 & 31783 & 29 & 6 &  MinerRay, SEISMIC 32-bit \\
 \hline
\end{grouptable}

%\end{adjustbox}

%\includegraphics[width=0.12\textwidth]{plots/heats/24aae13ae29d012fdf36cacc6871640f6883f07a0d42eea40cfe277950ca16c9.wasm.0.pdf}
%\includegraphics[width=0.12\textwidth]{plots/heats/24aae13ae29d012fdf36cacc6871640f6883f07a0d42eea40cfe277950ca16c9.wasm.1.pdf}
%\includegraphics[width=0.12\textwidth]{plots/heats/24aae13ae29d012fdf36cacc6871640f6883f07a0d42eea40cfe277950ca16c9.wasm.2.pdf}
%\includegraphics[width=0.12\textwidth]{plots/heats/24aae13ae29d012fdf36cacc6871640f6883f07a0d42eea40cfe277950ca16c9.wasm.3.pdf}
%\includegraphics[width=0.12\textwidth]{plots/heats/24aae13ae29d012fdf36cacc6871640f6883f07a0d42eea40cfe277950ca16c9.wasm.4.pdf}
%\includegraphics[width=0.12\textwidth]{plots/heats/24aae13ae29d012fdf36cacc6871640f6883f07a0d42eea40cfe277950ca16c9.wasm.5.pdf}
%\includegraphics[width=0.12\textwidth]{plots/heats/24aae13ae29d012fdf36cacc6871640f6883f07a0d42eea40cfe277950ca16c9.wasm.6.pdf}
%\includegraphics[width=0.12\textwidth]{plots/heats/24aae13ae29d012fdf36cacc6871640f6883f07a0d42eea40cfe277950ca16c9.wasm.7.pdf}


%\begin{adjustbox}{width=1\textwidth}
{
    \centering
    \begin{grouptable}{G4}
    24aae13a   & 62458 & 28339 & 37 & 4 &  SEISMIC \\
    \hline
    000415b2   
%    cryptonight obfuscated TODO check, this can be possibly merge with another group 
& 62466 & 28339 & 37 & 3  & SEISMIC \\
\hline
    \end{grouptable}
}



\begin{grouptable}{G5} 
643116ff   & 73010 & 31866 &  & 6 & MinerRay  \\
\hline
\end{grouptable}


\begin{grouptable} {G6}
    006b2fb6   & 87502 & 39544 & 90 & 4 & \url{https://github.com/deepwn/deepMiner} \\
    \hline
\end{grouptable}




\begin{grouptable}{G7}
15b86a25   & 100755 & 45881 & 79 & 4 &  MinerRay \\
\hline
\end{grouptable}


\begin{grouptable}{G8}
4cbdbbb1  
%NFWebMiner add to the description
% https://minero.cc/
& 104666 & 47916 & 62 & 3 & \url{https://github.com/wenhao1006/SEISMIC/tree/master/NFWebMiner}  \\
\hline
\child 119c53eb  & 137320 & 67069 & 79 & 2   & \url{https://github.com/wenhao1006/SEISMIC/tree/master/NFWebMiner}  \\
\hline
\end{grouptable}

\begin{grouptable}{G9}
f0b24409 & 77572 & 34918 & 59 & 2 & MinerRay   \\
\hline
c1be4071 & 77572 & 34918 & 59 & 2 & MinerRay    \\
\hline
a74a7cb8 & 77572 & 34918 & 59 & 2 & MinerRay    \\
\hline
a27b45ef & 77572 & 34918 & 59 & 2 & MinerRay     \\
\hline
6b8c7899 & 77572 & 34918 & 59 & 2 & MinerRay   \\
\hline
68ca7c0e & 77572 & 34918 & 59 & 2 & MinerRay     \\
\hline
65debcbe & 77572 & 34918 & 59 & 2 & MinerRay    \\
\hline
5bc53343 & 77572 & 34918 & 59 & 2 & MinerRay    \\
\hline
59955b4c & 77572 & 34918 & 59 & 2 & MinerRay    \\
\hline
\end{grouptable}


\begin{grouptable}{G10}
942be4f7    & 103520 & 46208 & 79 & 4 & MinerRay \\
\hline
\end{grouptable}

\begin{grouptable}{G11}
fb15929f   & 77054 & 33562 & 112 & 4 &  MinerRay  \\
\hline
\end{grouptable}


\begin{grouptable}{G12}
7c36f462   & 121931 & 55839 & 79 & 4 &  MinerRay \\
\hline
\end{grouptable}



\begin{grouptable}{G13}
89a3645c   & 75003 & 34134 & 58 & 2 &  MinerRay \\
\hline
\end{grouptable}

\begin{grouptable}{G14} 
dceaf65b    
% cryptonight-(v1|v7)  Check that this is packaged with multiple versions
& 77575 & 34901 & 58 & 2 &   MinerRay  \\
\hline

089dd312   
% cryptonight-(v1|v7)  Check that this is packaged with multiple versions
& 79883 & 34989 & 58 & 2 & MinerRay,  \live \url{http://theroyalforums.com},  \live \url{http://prylive.com.meta}  \\
\hline
\end{grouptable} 

\begin{grouptable}{G15}
e09c32c5  
%cryptonight (only \_cryptonight\_hash function) Check this 
& 71955 & 32416 & 46 & 1 & MinerRay  \\
\hline
\end{grouptable}



==> old/table_rq1.old.tex <==

\renewcommand\arraystretch{1.00}
\begin{adjustbox}{width=1\linewidth}
    \begin{tabular}{lrrr | lrrr | lrrr}
        \toprule
         \textbf{hash} &  \textbf{\#D}  &  \textbf{Max. \#evaded} & & \textbf{hash} &  \textbf{\#D}  &  \textbf{Max. \#evaded} &   & \textbf{hash} &  \textbf{\#D}  &  \textbf{Max. \#evaded} & \\
        \hline
47d29959 &                 31 &             {\color{gray} 26} &          & 
9d30e7f0 &                 30 &            {\color{gray} 24 } &          & 
8ebf4e44 &                 26 &             {\color{gray} 21} &          \\

\toprule
         &  &    & \textbf{Mean \#trans.} &  &   &   & \textbf{Mean \#trans.}  &  &   &   & \textbf{Mean \#trans.} \\
         
\hline 
dc11d82d &                 20 &              &  355 & 
0d996462 &                 19 &              &  401 & 
a32a6f4b &                 18 &              &  635 \\


fbdd1efa &                 18 &              &  310 & 
d2141ff2 &                  9 &               &  461 & 
aafff587 &                  6 &               &  484 \\


046dc081 &                  6 &               &  404 & 
643116ff &                  6 &               &  144 & 
15b86a25 &                  4 &               &  253 \\



006b2fb6 &                  4 &               &  282 & 
942be4f7 &                  4 &               &  200 & 
7c36f462 &                  4 &               &  236 \\


fb15929f &                  4 &               &  297 & 
24aae13a &                  4 &               &  252 & 
000415b2 &                  3 &               &  302 \\

4cbdbbb1 &                  3 &               &  295 & 
65debcbe &                  2 &               &  131 & 
59955b4c &                  2 &               &  130 \\


89a3645c &                  2 &               &  431 &
a74a7cb8 &                  2 &               &  124 &
119c53eb &                  2 &               &  104 \\

089dd312 &                  2 &               &  153 &
c1be4071 &                  2 &               &  130 &
dceaf65b &                  2 &               &  140 \\

6b8c7899 &                  2 &               &  143 &
a27b45ef &                  2 &               &  145 &
68ca7c0e &                  2 &               &  137 \\

f0b24409 &                  2 &               &  127 &
5bc53343 &                  2 &               &  118 &
e09c32c5 &                  1 &               &  120 \\
    \end{tabular}
\end{adjustbox}

==> old/table_rq3-.bck.tex <==


\todo{Swap correctness and h/s}
\todo{Fix table 4}

\renewcommand\arraystretch{0.95}
\begin{adjustbox}{width=1\linewidth}
  \begin{tabular}{c | cc || c | cc}

        \toprule
           ID &  \multicolumn{2}{c||}{Baseline algorithm} & \multicolumn{3}{c}{MCMC algorithm} \\
         \hline
          & h/s & correct. \% & $\sigma$ & h/s & correct. \% \\
         \hline

        \multirow{11}{*}{\shortstack[l]{0d996462 \\ \\ Original h/s: 64}} 
  & 27 (2.37) & 100 \% & $\sigma=0.01$ & 55 (1.16) & 100\% \\
 & 24 (2.67) & 100 \% \\
 & 26 (2.46) & 100 \% \\
 & 25 (2.56) & 100 \% \\
 & 24 (2.67) & 100 \% \\
 & 55 (1.16) & 100 \% \\
 & 102 (\textbf{0.63}) & 100 \% \\
 & 23 (2.78) & 100 \% \\
 & 30 (2.13) & 100 \% \\
 & 27 (2.37) & 100 \% \\
 & 26 (2.46) & 100 \% \\

        \hline
        \multirow{10}{*}{\shortstack[l]{a32a6f4b \\ \\ Original h/s: 26}} 
  & 24 (1.08) & 100 \% & $\sigma=0.01$ & 26 (\textbf{1.00}) & 100\% \\
 & 24 (1.08) & 100 \% \\
 & 26 (\textbf{1.00}) & 100 \% \\
 & 25 (1.04) & 100 \% \\
 & 23 (1.13) & 100 \% \\
 & 26 (\textbf{1.00}) & 100 \% \\
 & 24 (1.08) & 100 \% \\
 & 26 (\textbf{1.00}) & 100 \% \\
 & 25 (1.04) & 100 \% \\
 & 25 (1.04) & 100 \% \\

        \hline
    

        \multirow{8}{*}{\shortstack[l]{fbdd1efa \\ \\ Original h/s: 19}} 
  & 26 (\textbf{0.73}) & 100 \% & $\sigma=0.01$ & 28 (\textbf{0.68}) & 100\% \\
 & 25 (\textbf{0.76}) & 100 \% \\
 & 25 (\textbf{0.76}) & 100 \% \\
 & 25 (\textbf{0.76}) & 100 \% \\
 & 25 (\textbf{0.76}) & 100 \% \\
 & 25 (\textbf{0.76}) & 100 \% \\
 & 25 (\textbf{0.76}) & 100 \% \\
 & 26 (\textbf{0.73}) & 100 \% \\

        \hline
    
        \multirow{9}{*}{\shortstack[l]{d2141ff2 \\ \\ Original h/s: 72}} 
  & 54 (1.33) & 100 \% & $\sigma=0.3$ & 61 (1.18) & 100\% \\
 & 55 (1.31) & 100 \% & $\sigma=0.01$ & 58 (1.24) & 100\% \\
 & 56 (1.29) & 100 \% \\
 & 57 (1.26) & 100 \% \\
 & 53 (1.36) & 100 \% \\
 & 57 (1.26) & 100 \% \\
 & 56 (1.29) & 100 \% \\
 & 55 (1.31) & 100 \% \\
 & 53 (1.36) & 100 \% \\

        \hline
    
        \multirow{9}{*}{\shortstack[l]{046dc081 \\ \\ Original h/s: 61}} 
  & 55 (1.11) & 100 \% & $\sigma=0.3$ & 62 (\textbf{0.98}) & 100\% \\
 & 60 (1.02) & 100 \% & $\sigma=0.01$ & 58 (1.05) & 100\% \\
 & 57 (1.07) & 100 \% \\
 & 59 (1.03) & 100 \% \\
 & 62 (\textbf{0.98}) & 100 \% \\
 & 55 (1.11) & 100 \% \\
 & 60 (1.02) & 100 \% \\
 & 50 (1.22) & 100 \% \\
 & 58 (1.05) & 100 \% \\

        \hline
    
        \multirow{5}{*}{\shortstack[l]{006b2fb6 \\ \\ Original h/s: 8}} 
  & 7 (1.14) & 100 \% & $\sigma=0.01$ & 6 (1.33) & 100\% \\
 & 6 (1.33) & 100 \% & $\sigma=0.3$ & 8 \textbf{(1.00)} & 100\% \\
 & 4 (2.00) & 100 \% \\
 & 6 (1.33) & 100 \% \\
 & 9 (\textbf{0.89}) & 100 \% \\

        \hline
    
    
    
    \end{tabular}

\end{adjustbox}


==> snippet1.tex <==

\lstdefinestyle{watcode}{
  numbers=none,
  stepnumber=1,
  numbersep=10pt,
  tabsize=4,
  showspaces=false,
  breaklines=true, 
  showstringspaces=false,
    moredelim=**[is][{\btHL[fill=black!10]}]{`}{`},
    moredelim=**[is][{\btHL[fill=celadon!40]}]{!}{!}
}

{\captionsetup{width=0.45\linewidth}
\noindent\begin{minipage}[b]{0.45\linewidth}
    \lstset{
        language=WAT,
        style=watcode,
        basicstyle=\footnotesize\ttfamily,
        columns=fullflexible,
        breaklines=true}
        \begin{lstlisting}[label=example:block1,caption={Original piece of code for the \texttt{089a3645c} WebAssembly binary.},frame=b, captionpos=b]{Name}
...
i32.const x
...
        \end{lstlisting}
        \vspace{0.26cm}
   \end{minipage}\hfill%
\noindent\begin{minipage}[b]{0.45\linewidth}
    \lstset{
        language=WAT,
                        style=watcode,
        basicstyle=\footnotesize\ttfamily,
                        columns=fullflexible,
                        breaklines=true}
        
        \begin{lstlisting}[label=example:block2,caption={Peephole mutations of \autoref{example:block1}. Only with this mutation VirusTotal passed from 2 initial detectors to 0 in our experiments.},frame=b, captionpos=b]{Name}
...
!i32.const y!
!i32.const (x - y)!
!i32.add!
...
        \end{lstlisting}
\end{minipage}
}


==> snippets/function_position_snippet.tex <==
   \lstset{
        language=WAT,
        style=nccode,
        basicstyle=\footnotesize\ttfamily,
        columns=fullflexible,
        breaklines=true
    }
    
    \begin{minipage}{\linewidth}
        \footnotesize
        \centering
        \lstset{numbers=none}
        \noindent\begin{minipage}[t]{.50\linewidth}
        \begin{lstlisting}[xleftmargin=1em,escapechar=?]
(_emcc... (func `57`))
(_errno... (func `62`))
            \end{lstlisting}
        \end{minipage}\hfill
        \noindent\begin{minipage}[t]{.50\linewidth}
    \begin{lstlisting}[xleftmargin=1em,escapechar=?]
(_emcc... (func !63!))
(_errno... (func !61!))
        \end{lstlisting}
            \end{minipage}
    \end{minipage}

==> snippets/instrumentation.tex <==
   \lstset{
        language=WAT,
        style=nccode,
        basicstyle=\footnotesize\ttfamily,
        columns=fullflexible,
        breaklines=true
    }
    
    \begin{minipage}{\linewidth}
        \footnotesize
        \centering
        \lstset{numbers=none}
        \noindent\begin{minipage}[t]{1\linewidth}
        \begin{lstlisting}[xleftmargin=1em,escapechar=?]
  global.get X
  (i64|i32).const 1
  (i64|i32).add
  global.set X
  ; instruction to instrument
            \end{lstlisting}
        \end{minipage}\hfill
        \noindent
    \end{minipage}

==> snippets/multiple_hashing.tex <==
   \lstset{
        language=WAT,
        style=nccode,
        basicstyle=\footnotesize\ttfamily,
        columns=fullflexible,
        breaklines=true
    }
    
    \begin{minipage}{\linewidth}
        \footnotesize
        \centering
        \lstset{numbers=none}
        \noindent\begin{minipage}[t]{1\linewidth}
        \begin{lstlisting}[xleftmargin=1em,escapechar=?]
(export "_cryptonight_hash_variant_0" ...)
(export "_cryptonight_hash_variant_1" ...)
            \end{lstlisting}
        \end{minipage}\hfill
        \noindent
    \end{minipage}

==> snippets/obfuscation.tex <==
   \lstset{
        language=WAT,
        style=nccode,
        basicstyle=\footnotesize\ttfamily,
        columns=fullflexible,
        breaklines=true
    }
    
    \begin{minipage}{\linewidth}
        \footnotesize
        \centering
        \lstset{numbers=none}
        \noindent\begin{minipage}[t]{.50\linewidth}
        \begin{lstlisting}[xleftmargin=1em,escapechar=?]
`_i_want_hash`(f. 19)
`_i_want_create`(f. 17)
`_i_want_destroy`(f. 18) 
            \end{lstlisting}
        \end{minipage}\hfill
        \noindent\begin{minipage}[t]{.50\linewidth}
    \begin{lstlisting}[xleftmargin=1em,escapechar=?]
!obfuscated1! (f. 19)
!obfuscated2! (f. 17)
!obfuscated3! (f. 18)
        \end{lstlisting}
            \end{minipage}
    \end{minipage}

==> snippets/obfuscation2.tex <==
   \lstset{
        language=WAT,
        style=nccode,
        basicstyle=\footnotesize\ttfamily,
        columns=fullflexible,
        breaklines=true
    }
    
    \begin{minipage}{\linewidth}
        \footnotesize
        \centering
        \lstset{numbers=none}
        \noindent\begin{minipage}[t]{.50\linewidth}
        \begin{lstlisting}[xleftmargin=1em,escapechar=?]
_`XOuJTMJpKnE`_create (func 46)
_`XOuJTMJpKnE`_destroy (func 45)
_`XOuJTMJpKnE`_hash (func 44)
            \end{lstlisting}
        \end{minipage}\hfill
        \noindent\begin{minipage}[t]{.50\linewidth}
    \begin{lstlisting}[xleftmargin=1em,escapechar=?]
_!sRjBEbREsTx!_create (func 46)
_!sRjBEbREsTx!_destroy (func 45)
_!sRjBEbREsTx!_hash (func 44)
        \end{lstlisting}
            \end{minipage}
    \end{minipage}

==> table_rq3.2.tex <==


\renewcommand\arraystretch{1.2}
\begin{adjustbox}{width=1\linewidth}
  \begin{tabular}{c c | cr | cr | cr || cr | cr | cr}

        \toprule
           Hash &  Original h/s & \multicolumn{6}{c||}{Baseline algorithm} & \multicolumn{6}{c}{MCMC algorithm} \\
         \hline
           & & correct. \% & h/s & correct. \% & h/s & correct. \% & h/s 
        & correct. \% & h/s & correct. \% & h/s & correct. \% & h/s 
           \\
        \toprule
        0d996462  & 64 & 100 \% & 23(2.78) & 100 \% & 26(2.46)  & 100 \% & 102(\textbf{0.63})   & 100\% & 60 (1.06)  & 100\% & 61 (1.05)  & 100\% & 61 (1.05)  \\

        \hline
    

        \hline
        a32a6f4b  & 26 & 100 \% & 23(1.13) & 100 \% & 25(1.04)  & 100 \% & 26(\textbf{1.00})   & 100\% & 27 (\textbf{0.96})  & 100\% & 26 (\textbf{0.97})  & 100\% & 26 (\textbf{1.00})  \\

        \hline
    

        \hline
        fbdd1efa  & 19 & 100 \% & 25(\textbf{0.76}) & 100 \% & 25(\textbf{0.76})  & 100 \% & 26(\textbf{0.73})   & 100\% & 28 (\textbf{0.67})  & 100\% & 30 (\textbf{0.62})  & 100\% & 28 (\textbf{0.68})  \\

        \hline
    

        \hline
        d2141ff2  & 72 & 100 \% & 53(1.36) & 100 \% & 55(1.31)  & 100 \% & 57(1.26)   & 100\% & 59 (1.20)  & 100\% & 61 (1.18)  & 100\% & 58 (1.24)  \\

        \hline
    

        \hline
        046dc081  & 61 & 100 \% & 50(1.22) & 100 \% & 58(1.05)  & 100 \% & 62(\textbf{0.98})   & 100\% & 60 (1.02)  & 100\% & 62 (\textbf{0.98})  & 100\% & 58 (1.05)  \\

        \hline
    

        \hline
        006b2fb6  & 8 & 100 \% & 4(2.00) & 100 \% & 6(1.33)  & 100 \% & 9(\textbf{0.89})   & 100\% & 6 (1.25)  & 100\% & 7 (1.10)  & 100\% & 6 (1.33)  \\
        
    \end{tabular}

\end{adjustbox}


==> table_rq3.3.tex <==


\renewcommand\arraystretch{1.2}
\begin{adjustbox}{width=1\linewidth}
  \begin{tabular}{c c | cr  cr  cr || cr  cr  cr}

        \toprule
           Hash &  Original h/s & \multicolumn{6}{c||}{Baseline algorithm} & \multicolumn{6}{c}{MCMC algorithm} \\
         \hline


        \hline
        0d996462 & 116.0    & 100\% & 25 (4.64)  & 100\% & 24 (4.83)  & 100\% & 26 (4.46)   & 100\% & 116 (\textbf{1.00})  & 100\% & 70 (1.66)  & 100\% & 67 (1.73)  \\
                 &  & 100\% & 116 (\textbf{1.00})  & 100\% & 110 (1.05)  & 100\% & 30 (3.87)   & 100\% & 110 (1.05)  & 100\% & 76 (1.53)  & 100\% & 60 (1.93)  \\
                 &  & 100\% & 55 (2.11)  & 100\% & 27 (4.30)  & 100\% & 23 (5.04)   & 100\% & 86 (1.35)  & 100\% & 60 (1.93)  & 100\% & 72 (1.61)  \\
                 &  & 100\% & 27 (4.30)   & & & & &  100\% & 76 (1.53)  \\
                
        \hline
    

        \hline
        a32a6f4b & 48.0  &  100\% & 25 (1.92)  & 100\% & 24 (2.00)  & 100\% & 24 (2.00)   & 100\% & 26 (1.85)  & 100\% & 45 (1.07)  & 100\% & 41 (1.17)  \\
                 &  & 100\% & 26 (1.85)  & 100\% & 25 (1.92)  & 100\% & 26 (1.85)   & 100\% & 46 (1.04)  & 100\% & 41 (1.17)  & 100\% & 45 (1.07)  \\
                 &  & 100\% & 26 (1.85)  & 100\% & 24 (2.00)  & 100\% & 25 (1.92)   & 100\% & 44 (1.09)  & 100\% & 42 (1.14)  & 100\% & 45 (1.07)  \\
                 &  & 100\% & 23 (2.09)   & &&&& 100\% & 45 (1.07)  \\
                
        \hline
    

        \hline
        fbdd1efa & 37.0    & 100\% & 25 (1.48)  & 100\% & 25 (1.48)  & 100\% & 25 (1.48)   & 100\% & 28 (1.32)  & 100\% & 47 (\textbf{0.79})  & 100\% & 48 (\textbf{0.77})  \\
                 &  & 100\% & 25 (1.48)  & 100\% & 26 (1.42)  & 100\% & 26 (1.42)   & 100\% & 47 (\textbf{0.79})  & 100\% & 47 (\textbf{0.79})  & 100\% & 53 (\textbf{0.70})  \\
                 &  & 100\% & 25 (1.48)  & 100\% & 25 (1.48)  & 100\% & 25 (1.48)   & 100\% & 48 (\textbf{0.77})  & 100\% & 48 (\textbf{0.77})  & 100\% & 49 (\textbf{0.76})  \\
                 &  & 100\% & 25 (1.48)    & &&& & 100\% & 47 (\textbf{0.79})  \\
                
        \hline
    

        \hline
        d2141ff2 & 113.0   & 100\% & 54 (2.09)  & 100\% & 55 (2.05)  & 100\% & 55 (2.05)   & 100\% & 107 (1.06)  & 100\% & 107 (1.06)  & 100\% & 107 (1.06)  \\
                 &  & 100\% & 57 (1.98)  & 100\% & 56 (2.02)  & 100\% & 56 (2.02)   & 100\% & 109 (1.04)  & 100\% & 106 (1.07)  & 100\% & 100 (1.13)  \\
                 &  & 100\% & 57 (1.98)  & 100\% & 53 (2.13)  & 100\% & 53 (2.13)   & 100\% & 101 (1.12)  & 100\% & 100 (1.13)  & 100\% & 107 (1.06)  \\
                 &  & 100\% & 55 (2.05)    & &&& & 100\% & 107 (1.06)  \\
                
        \hline
    

        \hline
        046dc081 & 118.0   & 100\% & 58 (2.03)  & 100\% & 60 (1.97)  & 100\% & 59 (2.00)   & 100\% & 118 (\textbf{1.00})  & 100\% & 120 (\textbf{0.98})  & 100\% & 119 (\textbf{0.99})  \\
                 &  & 100\% & 60 (1.97)  & 100\% & 55 (2.15)  & 100\% & 62 (1.90)   & 100\% & 120 (\textbf{0.98})  & 100\% & 116 (1.02)  & 100\% & 120 (\textbf{0.98})  \\
                 &  & 100\% & 55 (2.15)  & 100\% & 50 (2.36)  & 100\% & 57 (2.07)   & 100\% & 119 (\textbf{0.99})  & 100\% & 120 (\textbf{0.98})  & 100\% & 119 (\textbf{0.99})  \\
                 &  & 100\% & 55 (2.15)    & &&& & 100\% & 120 (\textbf{0.98})  \\
                
        \hline
    

        \hline
        006b2fb6 & 8.0   & 100\% & 7 (1.14)  & 100\% & 6 (1.33)  & 100\% & 4 (2.00)   & 100\% & 6 (1.33)  & 100\% & 6 (1.33)  & 100\% & 6 (1.33)  \\
                 &  & 100\% & 9 (\textbf{0.89})  & 100\% & 6 (1.33)  & 100\% & 4 (2.00)   & 100\% & 6 (1.33)  & 100\% & 6 (1.33)  & 100\% & 6 (1.33)  \\
                 &  & 100\% & 4 (2.00)  & 100\% & 6 (1.33)  & 100\% & 4 (2.00)   & 100\% & 8 (\textbf{1.00})  & 100\% & 9 (\textbf{0.88})  & 100\% & 6 (1.33)  \\
                 &  & 100\% & 6 (1.33)    & &&&& 100\% & 6 (1.33)  \\
                
        \hline
    
        
    \end{tabular}

\end{adjustbox}


==> table_rq3.tex <==

\large

\renewcommand\arraystretch{1.20}
\begin{adjustbox}{width=1\linewidth}
  \begin{tabular}{l | l  | lllll lllll | lll}
  ID & Original & \multicolumn{10}{c|}{Baseline algorithm variants} & \multicolumn{3}{c}{ MCMC algorithm variants} \\
  & & \multicolumn{10}{c |}{} & $\sigma$=0.01 & $\sigma$=0.3 & $\sigma$=1.1 \\
  \hline
  
0d996462 & 64.0 h/s &  27.0(2.37) & 24.0(2.67) & 26.0(2.46) & 25.0(2.56) & 24.0(2.67) & 55.0(1.16) & 102.0(\textbf{0.63}) & 23.0(2.78) & 30.0(2.13) & 27.0(2.37) & 64.0\textbf{(1.0)} && \\

a32a6f4b & 26.0 h/s &  24.0(1.08) & 24.0(1.08) & 26.0(\textbf{1.00}) & 25.0(1.04) & 23.0(1.13) & 26.0(\textbf{1.00}) & 24.0(1.08) & 26.0(\textbf{1.00}) & 25.0(1.04) & 25.0(1.04) & 26.0(\textbf{1.0}) && \\

fbdd1efa & 19.0 h/s &  26.0(\textbf{0.73}) & 25.0(\textbf{0.76}) & 25.0(\textbf{0.76}) & 25.0(\textbf{0.76}) & 25.0(\textbf{0.76}) & 25.0(\textbf{0.76}) & 25.0(\textbf{0.76}) & 26.0(\textbf{0.73}) & & & 28.0(\textbf{0.68}) && \\

d2141ff2 & 72.0 h/s &  54.0(1.33) & 55.0(1.31) & 56.0(1.29) & 57.0(1.26) & 53.0(1.36) & 57.0(1.26) & 56.0(1.29) & 55.0(1.31) & 53.0(1.36) & & 58.0(1.2) & 61.0(1.2) & \\

046dc081 & 61.0 h/s &  55.0(1.11) & 60.0(1.02) & 57.0(1.07) & 59.0(1.03) & 62.0(\textbf{0.98}) & 55.0(1.11) & 60.0(1.02) & 50.0(1.22) & 58.0(1.05) & & 58.0(1.1) & 62.0(\textbf{0.98}) & \\

006b2fb6 & 8.0 h/s &  7.0(1.14) & 6.0(1.33) & 4.0(2.00) & 6.0(1.33) & 9.0(\textbf{0.89}) & & & & & & 6.0(1.3) & 6.0(1.3)& \\
 
    \end{tabular}

\end{adjustbox}

==> table_rq4.tex <==


\renewcommand\arraystretch{1.20}
%\begin{adjustbox}{width=1\linewidth}
  \begin{tabular}{lr|rccc|rccc}
\textbf{Hash} &  \textbf{\#D}  & \multicolumn{4}{c}{No. Stacked mutations} \\
 &  &  BS & \multicolumn{3}{c}{MCMC} \\
 & & & $\sigma$=01 & $\sigma$=0.3 & $\sigma$=1.1 & & \\
\hline
47d29959 & 31 &  &  &  &  \\
9d30e7f0 & 30 &  &  &  &  \\
8ebf4e44 & 26 &  &  &  &  \\
dc11d82d & 20 & 355 & 444 &  &  \\
0d996462 & 19 & 401 & 696 &  &  \\
a32a6f4b & 18 & 635 & 621 &  &  \\
fbdd1efa & 18 & 310 & 725 &  &  \\
d2141ff2 & 9 & 461 & 775 & 603 &  \\
aafff587 & 6 & 484 &  & 228 & 76 \\
046dc081 & 6 & 404 & 397 & 158 &  \\
643116ff & 6 & 144 & 436 & 484 &  \\
15b86a25 & 4 & 253 & 207 & 186 & 109 \\
006b2fb6 & 4 & 282 & 379 & 500 &  \\
942be4f7 & 4 & 200 & 200 & 195 & 142 \\
7c36f462 & 4 & 236 & 221 &  &  \\
fb15929f & 4 & 297 &  & 446 &  \\
24aae13a & 4 & 252 & 398 & 286 &  \\
000415b2 & 3 & 302 & 373 & 19 &  \\
4cbdbbb1 & 3 & 295 & 204 & 62 & 168 \\
65debcbe & 2 & 131 & 33 & 31 & 31 \\
59955b4c & 2 & 130 & 33 & 33 & 33 \\
89a3645c & 2 & 431 & 318 & 152 & 1 \\
a74a7cb8 & 2 & 124 & 33 & 33 & 33 \\
119c53eb & 2 & 104 & 44 & 352 & 7 \\
089dd312 & 2 & 153 & 166 & 149 & 18 \\
c1be4071 & 2 & 130 & 33 & 33 & 33 \\
dceaf65b & 2 & 140 & 165 & 165 & 48 \\
6b8c7899 & 2 & 143 & 33 & 33 & 33 \\
a27b45ef & 2 & 145 & 33 & 30 & 33 \\
68ca7c0e & 2 & 137 & 33 & 121 & 15 \\
f0b24409 & 2 & 127 & 11 & 33 & 11 \\
5bc53343 & 2 & 118 & 33 & 33 & 33 \\
e09c32c5 & 1 & 120 & 478 & 595 &  \\
\end{tabular}




%\end{adjustbox}
